Efficient decomposition of unitary matrices in quantum circuit compilers

Unitary decomposition is a widely used method to map quantum algorithms to an arbitrary set of quantum gates. Efficient implementation of this decomposition allows for translation of bigger unitary gates into elementary quantum operations, which is key to executing these algorithms on existing quantum computers. The decomposition can be used as an aggressive optimization method for the whole circuit, as well as to test part of an algorithm on a quantum accelerator. For selection and implementation of the decomposition algorithm, perfect qubits are assumed. We base our decomposition technique on Quantum Shannon Decomposition which generates O((3/4)*4^n) controlled-not gates for an n-qubit input gate. The resulting circuits are up to 10 times shorter than other methods in the field. When comparing our implementation to Qubiter, we show that our implementation generates circuits with half the number of CNOT gates and a third of the total circuit length. In addition to that, it is also up to 10 times as fast. Further optimizations are proposed to take advantage of potential underlying structure in the input or intermediate matrices, as well as to minimize the execution time of the decomposition.

==> B_Example.tex <==
\vspace{2em}
\textbf{A "simple" decomposition example} \\
To illustrate what unitary decomposition entails, I will use the example of a general two-qubit gate. The 4 by 4 unitary matrix has been randomly generated. Our example matrix is called "U", for "Unitary", and is shown below\footnote{\lstinline{j} is the python representation for the imaginary number $i = \sqrt{-1}$}:
%With the code shown in \cref{lst:gen_unitary}, generalized unitary matrices can be generated. 
%From this code, a unitary matrix is generated, which could look like this for a two qubit gate, called "U":  

\begin{center}
\begin{minipage}[H]{0.7\textwidth}
\begin{lstlisting}[basicstyle=\small\ttfamily\color{black}, numbers=none]
U = [ 0.077+0.669j, -0.234+0.315j,  0.138+0.428j, -0.39 -0.196j, 
     -0.202+0.208j,  0.757+0.308j, -0.451+0.143j,  0.032+0.153j,
     -0.533+0.091j, -0.094+0.05j ,  0.451+0.192j,  0.192+0.648j,  
      0.412+0.029j, -0.393+0.111j, -0.494+0.299j,  0.407+0.404j]
\end{lstlisting}
\end{minipage}
\end{center}
The circuit representation of this matrix would be:
\begin{equation*}
\Qcircuit @C=1em @R=.7em {
&\multigate{1}{U}   & \qw   \\
&\ghost{U}          &\qw     }
\end{equation*}
This matrix is decomposed with the following commands in OpenQL:
\begin{center}
\begin{minipage}[H]{0.7\textwidth}
\begin{lstlisting}[morekeywords={Unitary, decompose, add_kernel},basicstyle=\small\ttfamily\color{black}]
  import openql.openql as ql
  # OpenQL preamble
  unitary = ql.Unitary('u1', U)
  unitary.decompose()
\end{lstlisting}
\end{minipage}
\end{center}


\subsection{Cosine Sine Decomposition}
When the program is compiled, the matrix is decomposed in several steps. The first is the Cosine Sine Decomposition. This decomposition calculates three matrices, and the product of these matrices is the original matrix $U$.%
\begin{align*}
U = R_{12}*F^1_0(R_{y})*L_{12}
\end{align*}
{\small
\begin{align*}\renewcommand*{\arraystretch}{1.2}
R_{12} = &\begin{pmatrix} 0.517 + 0.658j & -0.131 + 0.532j & 0  & 0 \\
 -0.504 + 0.214j  &0.731 + 0.407j & 0 & 0\\
  0 & 0 & -0.581 + 0.340j & -0.644 + 0.364j \\
  0 & 0 & 0.780,+ -0.208j & -0.650 + 0.180j \end{pmatrix} \\[0.3em]
F^1_0(R_y) =  &\begin{pmatrix} C & S \\ -S & C \end{pmatrix} =  
\begin{pmatrix} 0.706+0j        &0&-0.708+0j &0 \\
0 &0.927+0j       &-0+-0j            &-0.374+-0j \\
0.708+0j &0&0.706277+0j        &0 \\ 
0            &0.374+0j&0 &0.927+0j \end{pmatrix} \\[0.3em]
L_{12} = &\begin{pmatrix} 0.886+0.330j      &-0.325+-0j  & 0 & 0\\
0.305+0.114j       &0.946+-0j  & 0 & 0\\
 0 & 0 & -0.863+-0.219j &0.444+-0.100j \\ 
 0 & 0 & 0.166+-0.424j &-0.086+-0.886j \end{pmatrix}
\end{align*}
}
Which looks like this in a quantum circuit:
\begin{equation*}
\Qcircuit @C=1em @R=.7em {
&\multigate{1}{U}   & \qw   & 
& &\qw &\multigate{1}{L_{12}} &\qw &\qw & \gate{R_y} &\qw & \multigate{1}{R_{12}} & \qw &\qw\\
   &\ghost{U}          &\qw    &\push{\rule{.3em}{0em}\raisebox{2.2em}{=}\rule{.3em}{0em}}
& &\qw &\ghost{U_{12}}        &\qw &\qw & \ctrlb{-1} &\qw & \ghost{V_{12}}  & \qw &\qw }
\end{equation*}
The $L_{12}$ and $R_{12}$ matrices represent two-qubit gates, where either the upper left matrix, or the lower right matrix gets applied to the lower qubit, depending on the value of the top qubit. This is called a multiplexor. The $F^1_0(R_y)$ gate is a multiplexed rotation-y gate with 1 control gate, applied to qubit 0. This gate rotates the qubit around the Y-axis with a different angle for each possible value of the controlling qubit(s).

\subsection{Singular Value Decomposition}
The general multiplexors $L_{12}$ and $R_{12}$ get decomposed using Singular Value Decomposition. This generates again three matrices per multiplexor, which result in the original matrix when they are multiplied:
\begin{align*}
    U_{12} &= ( I \otimes V_L )\cdot F^1_0(R_z)_L \cdot (I\otimes W_L)
\end{align*}%
{\small
\begin{align*}\renewcommand*{\arraystretch}{1.2}
I \otimes V_L &= \begin{pmatrix}0.0636+0.078j &-0.995+0j  & 0 & 0 \\
0.897+0.430j &0.091+-0.043j & 0 & 0\\
0 & 0&0.064+0.078j          &-0.995+0j\\
0 & 0&0.897+0.430j &0.091+-0.043j\end{pmatrix} \\[0.3em]
 V_L &= \begin{pmatrix}0.0636+0.078j  &-0.995+0j\\
0.897+0.430j &0.0911+-0.043j \end{pmatrix} \\
F^1_0(R_z)_L &= \begin{pmatrix} D & 0 \\ 0 & D^\dagger \end{pmatrix} = \begin{pmatrix} 0.682+0.731j &0  & 0 & 0\\
            0 &0.067+-0.998j  & 0 & 0\\
              0 & 0 &0.682-0.731j &0\\
              0 & 0 &0 &0.067+0.998j \end{pmatrix} \\[0.3em]
I\otimes W_L &= \begin{pmatrix} 0.219+-0.349j &0.285+-0.865j     & 0 & 0 \\
                                0.247+-0.877j &-0.013+0.411j   & 0 & 0 \\
                                0 & 0     &0.219+-0.349j    &0.285+-0.865j \\
                                0 & 0     & 0.247+-0.877j   &-0.019+0.411j \end{pmatrix}\\[0.3em]
W_L &= \begin{pmatrix}  0.219+-0.349j   &0.285+-0.865j \\
                    0.247+-0.877j   &-0.013+0.411j \end{pmatrix}
\end{align*}
}
As a quantum circuit, it now looks like this:

\begin{equation*}
\Qcircuit @C=1em @R=.7em {
&\qw &\multigate{1}{U}   & \qw   & 
& &\qw &\qw & \gate{(R_z)_L} &\qw & \gate{R_y} &\qw & \multigate{1}{R_{12}} & \qw &\qw\\
&\qw   &\ghost{U}          &\qw    &\push{\rule{.3em}{0em}\raisebox{2.2em}{=}\rule{.3em}{0em}}
& &\qw &\gate{W_L} & \ctrlb{-1} &\gate{V_L} & \ctrlb{-1} &\qw & \ghost{R_{12}}  & \qw &\qw }
\end{equation*}
As you can see, the 2-by-2 matrices $V_L$ and $W_L$ are single qubit gates on the lower qubit, while the multiplexed $R_z$ gate is applied to the upper qubit, just like the multiplexed $R_y$ gate. 

The same is then done for matrix $R_{12}$:
\begin{align*}
        R_{12} &= ( I \otimes V_R )\cdot F^1_0(R_{z})_R \cdot (I\otimes W_R)
\end{align*}
{\small
\begin{align*}\renewcommand*{\arraystretch}{1.2}
    I \otimes V_R &= \begin{pmatrix}0.938+0j  &0.310+-0.156j  & 0 & 0 \\
   0.183+-0.295j &-0.083+0.934j & 0 & 0\\
    0 & 0&0.938+0j  &0.310+-0.156j\\
    0 & 0&0.183+-0.295j &-0.083+0.934j\end{pmatrix} \\[0.3em]
     V_R &= \begin{pmatrix}0.938+0j  &0.310+-0.156j\\
  0.183+-0.295j &-0.083+0.934j \end{pmatrix} \\[0.3em]
    F^1_0(R_z)_R &= \begin{pmatrix} D & 0 \\ 0 & D^\dagger \end{pmatrix} = \begin{pmatrix}0.825+-0.566j &0  & 0 & 0\\
                0 &0.135+-0.991j  & 0 & 0\\
                  0 & 0 &0.825+0.566j &0\\
                  0 & 0 &0 &0.135+0.991j \end{pmatrix} \\[0.3em]
    I\otimes W_R &= \begin{pmatrix}-0.015+0.605j  &-0.536+0.589j   & 0 & 0 \\
                                    -0.691+0.397j   &0.593+0.116j  & 0 & 0 \\
                                    0 & 0     &-0.015+0.605j  &-0.536+0.589j\\
                                    0 & 0     & -0.691+0.397j   &0.593+0.116j \end{pmatrix}\\[0.3em]
 W_R &= \begin{pmatrix}  -0.015+0.605j  &-0.536+0.589j \\
                       -0.691+0.397j   &0.593+0.116j \end{pmatrix}
\end{align*}
}
So the complete circuit is now:
\begin{equation*}
\Qcircuit @C=1em @R=.7em {
 &\multigate{1}{U}   & \qw   & 
& &\qw &\qw & \gate{(R_z)_L} &\qw & \gate{R_y}           &\qw & \gate{(R_z)_R} & \qw &\qw\\
   &\ghost{U}          &\qw    &\push{\rule{.3em}{0em}\raisebox{2.2em}{=}\rule{.3em}{0em}}
& &\qw &\gate{W_L} & \ctrlb{-1} &\gate{V_L} & \ctrlb{-1} &\gate{W_R} & \ctrlb{-1}  & \gate{V_R} &\qw }
\end{equation*}

\subsection{Demultiplexing and ZYZ decomposition}
Before this circuit can be executed on a real quantum computer, two more steps need to happen. The first is to translate the multiplexed rotation gates into regular rotation gates and CNOTs. For a two-qubit gate, this means two CNOT gates and two rotation gates per multiplexed gate.%
\begin{align*}
    &F^1_0(R_y) = CNOT\cdot (I \otimes R_y(\theta_0)) \cdot CNOT \cdot  (I \otimes R_y(\theta_1)) \\
    &F^1_0(R_z) = CNOT\cdot (I \otimes R_z(\theta_0)) \cdot CNOT \cdot  (I \otimes R_z(\theta_1)) \\
\end{align*}%
Which makes the circuit the following, with 6 different angles $\theta$:
\begin{equation*}
\Qcircuit @C=0.5em @R=.7em {
 &\multigate{1}{U}   & \qw   & 
& &\qw &\qw & \targ & \gate{R_z(\theta_0)_L} & \targ & \gate{R_z(\theta_1)_L}  &\qw & \targ & \gate{R_y(\theta_0)} & \targ & \gate{R_y(\theta_1)}         &\qw & \targ & \gate{R_z(\theta_0)_R} & \targ & \gate{R_z(\theta_1)_R}  & \qw &\qw\\
   &\ghost{U}          &\qw    &\push{\rule{.3em}{0em}\raisebox{2.2em}{=}\rule{.3em}{0em}}
& &\qw &\gate{\scalebox{1.2}{$W_L$}} &\ctrl{-1} & \qw &\ctrl{-1} & \qw &\gate{\scalebox{1.2}{$V_L$}} &\ctrl{-1} & \qw &\ctrl{-1} & \qw  &\gate{\scalebox{1.2}{$W_R$}} &\ctrl{-1} & \qw &\ctrl{-1} & \qw & \gate{\scalebox{1.2}{$V_R$}} &\qw }
\end{equation*}
The angles for these rotation gates are found by solving the following equation, which follows from the set order of CNOTs:
\begin{align*}\renewcommand*{\arraystretch}{1.2}
    &\begin{pmatrix} 1 & 1 \\ 1 & -1\end{pmatrix}\begin{pmatrix} \theta_0 \\ \theta_1 \end{pmatrix} = \begin{pmatrix} \alpha_0 \\ \alpha_1 \end{pmatrix}\\
    &\begin{pmatrix}\alpha_0 \\ \alpha_1 \end{pmatrix}_{Ry} = 2\cdot arcsin(diag(S)) = 2\cdot arcsin\begin{pmatrix}-0.708 \\ -0.374 \end{pmatrix} \\
    &\begin{pmatrix}\alpha_0 \\ \alpha_1 \end{pmatrix}_{Rz} = -2j\cdot log(diag(D)) \\
    &\begin{pmatrix}\alpha_0 \\ \alpha_1 \end{pmatrix}_{Rz_L} = -2j \cdot log\begin{pmatrix}0.682+0.731j \\ 0.067-0.998j \end{pmatrix} \\
    &\begin{pmatrix}\alpha_0 \\ \alpha_1 \end{pmatrix}_{Rz_R} = -2j \cdot log\begin{pmatrix}0.825-0.566j\\ 0.135-0.991j \end{pmatrix}
\end{align*}
%\begin{align*}
%    Mux(r_y) = \begin{pmatrix} 1 & 0 & 0 & 0 \\0 & 0 & 0 & 1\\0 & 0 & 1 & 0 & 0\\0 & 1 & 0 & 0\end{pmatrix} 
%\end{align*}

The single qubit gates can be transformed into three rotation gates, like this:
\begin{align*}
    U(2) = R_z(\alpha)R_y(\beta)R_z(\gamma)
\end{align*}

\subsection{Final circuit}

So the total circuit, with the correct rotation angles in radians, is now the following circuit:  \footnote{The angles are rounded to two decimals because otherwise the circuit does not fit on the page. For the same reason, the circuit has been split into two lines.} 
{\small
\begin{align*}
&\Qcircuit @C=1em @R=1em {
&\multigate{1}{U}   & \qw   & 
& &&\qw &\qw   &\qw &\qw 
& \targ & \gate{R_z(0.68)} & \targ & \gate{R_z(2.32)}
 &\qw &\qw  &\qw \\
 &\ghost{U}          &\qw    &\push{\rule{.3em}{0em}\raisebox{2.2em}{=}\rule{.3em}{0em}}&
& &\qw &\gate{R_z(2.90)} &\gate{R_y(\text{-}0.85)} &\gate{R_z(\text{-}2.85)} 
& \ctrl{-1} & \qw & \ctrl{-1} 
 &\gate{R_z(4.03)} &\gate{R_y(\text{-}0.20)} &\gate{R_z(\text{-}0.45)} &\qw
 }\\
&\Qcircuit @C=1em @R=1em {
 & \targ & \gate{R_y(1.17)} & \targ & \gate{R_y(0.40)}      
 &\qw &\qw 
& \targ & \gate{R_z(2.04)} & \targ & \gate{R_z(0.83)}
 &\qw &\qw  &\qw \\
& \ctrl{-1} & \qw & \ctrl{-1}
 &\gate{R_z(3.86)} &\gate{R_y(\text{-}1.30)} &\gate{R_z(2.12)} 
& \ctrl{-1} & \qw & \ctrl{-1}
 &\gate{R_z(\text{-}0.47)} &\gate{R_y(\text{-}2.43)} &\gate{R_z(\text{-}1.02)} 
&\qw }
\end{align*}
}

All these operations are done by OpenQL, and all that is left is to apply this circuit to some qubits. That is done with the following code, after the one shown before:

\begin{center}
\begin{minipage}[H]{0.7\textwidth}
\begin{lstlisting}[morekeywords={Unitary, decompose, add_kernel},basicstyle=\small\ttfamily\color{black}]
 kernel.gate(unitary, [0,1])
 program.add_kernel(kernel)
 program.compile()
\end{lstlisting}
\end{minipage}
\end{center}

This compiles the circuit and the program into something that can be executed on a simulator or quantum accelerator, or into Quantum Assembly Language (QASM) as:
% \subsubsection{In OpenQL}
% As can be seen, this process has a lot of steps, and a two-qubit gate, with just 16 matrix entries, already results in 18 rotation gates and 6 CNOT gates. This number increases exponentially with the number of qubits the input matrix affects. Therefore, any human involvement in this decomposition will make it very error-prone. And because the resulting circuits are very long, very unclear and inconvenient to use. So ideally, the decomposition is handled by a computer algorithm implemented in the compiler, so that a user can just use arbitrary unitary gates in any algorithm without having to deal with the decomposition. 

% With the unitary decomposition implemented in OpenQL, the way to generate this circuit as quantum assembly language (QASM), is very simple. First the matrix is defined. This can also be the output of some algorithm or function. This matrix is added to a "Unitary" object, and decomposed. Then, the "Unitary" is added to the kernel in the same way as normal gates. 

% \begin{lstlisting}[language=Python, basicstyle=\small\ttfamily\color{black}, morekeywords={U, u_unitary}]
% U = [ 0.077+0.669j, -0.234+0.315j,  0.138+0.428j, -0.39 -0.196j, 
% -0.202+0.208j,  0.757+0.308j, -0.451+0.143j,  0.032+0.153j,
% -0.533+0.091j, -0.094+0.05j ,  0.451+0.192j,  0.192+0.648j,  
% 0.412+0.029j, -0.393+0.111j, -0.494+0.299j,  0.407+0.404j]
% u_unitary = ql.Unitary("Unitary",U)
% u_unitary.decompose()
% kernel.gate(u_unitary, [0,1])
% \end{lstlisting}
% OpenQL takes the matrix, goes through all the decomposition steps, and finally makes the same circuit. This circuit is printed as QASM:
\begin{center}
\begin{minipage}[H]{0.7\textwidth}
\begin{lstlisting}[basicstyle=\footnotesize]
version 1.0
# this file has been automatically generated by the OpenQL compiler please do not modify it manually.
qubits 2

.newKernel
    rz q[0], 2.898309
    ry q[0], -0.848687
    rz q[0], -2.853675
    rz q[1], 0.681902
    cnot q[0],q[1]
    rz q[1], 2.323443
    cnot q[0],q[1]
    rz q[0], 4.033960
    ry q[0], -0.201912
    rz q[0], -0.446115
    ry q[1], 1.169904
    cnot q[0],q[1]
    ry q[1], 0.403249
    cnot q[0],q[1]
    rz q[0], 3.857529
    ry q[0], -1.299610
    rz q[0], 2.115405
    rz q[1], 2.036688
    cnot q[0],q[1]
    rz q[1], 0.833905
    cnot q[0],q[1]
    rz q[0], 0.465892
    ry q[0], -2.432474
    rz q[0], -1.016344
\end{lstlisting}
\end{minipage}
\end{center}

\twocolumn
